Bridging Modalities: Enhancing Cross-Modality Hate Speech Detection with Few-Shot In-Context Learning

The widespread presence of hate speech on the internet, including formats such as text-based tweets and vision-language memes, poses a significant challenge to digital platform safety. Recent research has developed detection models tailored to specific modalities; however, there is a notable gap in transferring detection capabilities across different formats. This study conducts extensive experiments using few-shot in-context learning with large language models to explore the transferability of hate speech detection between modalities. Our findings demonstrate that text-based hate speech examples can significantly enhance the classification accuracy of vision-language hate speech. Moreover, text-based demonstrations outperform vision-language demonstrations in few-shot learning settings. These results highlight the effectiveness of cross-modality knowledge transfer and offer valuable insights for improving hate speech detection systems.

==> examples/cs2-p1-example1.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{p{\linewidth}}
\toprule

\textbf{\#\#\# EXAMPLE 1}\\ 
\textbf{Content:} A post containing 'because too many of them are ( ( ( white ) ) ) .'\\
\textbf{Answer:} Hateful\\
Rationale: Targeted Group: The post targets white individuals by implying that they are a problem or undesirable.\\

Derogatory Imagery/Language: The repeated use of the word "white" in parentheses suggests a derogatory and dismissive attitude towards white people.\\

Impact on Bias/Stereotypes: The post reinforces harmful stereotypes and prejudices against white people, potentially inciting fear and hostility towards them. It contributes to a divisive and exclusionary environment by implying that white individuals are a problem that needs to be addressed.\\

In summary, this post is hateful.\\ \\

\textbf{\#\#\# EXAMPLE 2}\\ 
\textbf{Content:} A post containing 'did you hear about the woman who got hit by a car ? police are questioning why she was out of the kitchen .'
\textbf{Answer:} Hateful\\
Rationale: Targeted Group: The post targets women, particularly those who are homemakers or stay-at-home mothers, by implying that they should be confined to the kitchen.\\

Derogatory Imagery/Language: The statement uses derogatory language by suggesting that women belong in the kitchen and should not be out in public.\\

Impact on Bias/Stereotypes: This post reinforces harmful stereotypes and prejudices against women, limiting their roles and opportunities in society. It perpetuates the idea that women's primary responsibility is in the home, and it could incite discrimination and exclusion against women who do not conform to these traditional gender roles.\\

In summary, this post is hateful.\\ \\

\textbf{\#\#\# EXAMPLE 3}\\ 
\textbf{Content:} A post containing 'take her money, fine her, and deport her dependents too.'\\
\textbf{Answer:} Hateful\\
Rationale: Targeted Group: The post targets immigrants, specifically those who have dependents, by suggesting that their family members should be punished alongside them.\\

Derogatory Imagery/Language: The statement uses dehumanizing language by treating immigrants and their dependents as if they are disposable or expendable.\\

Impact on Bias/Stereotypes: This post reinforces harmful stereotypes and prejudices against immigrants, suggesting that they are a burden on society and that their families should suffer as a result of their actions. It also contributes to an environment that doesn't respect or support the rights and well-being of immigrants and their families.\\

In summary, this post is hateful. \\ \\

\textbf{\#\#\# EXAMPLE 4}\\ 
\textbf{Content:} A post containing 'jared taylor on young'\\
\textbf{Answer:} Not Hateful\\
Rationale: Targeted Group: The post does not explicitly target a specific group with harmful intent.\\

Derogatory Imagery/Language: There is no derogatory language or imagery used in the post.\\

Impact on Bias/Stereotypes: The post does not perpetuate harmful stereotypes or prejudices against any group. It simply mentions a person's name, Jared Taylor, who is a known figure in certain political circles. However, it is essential to note that Jared Taylor is a controversial figure due to his views on race and ethnicity, which some may find offensive or discriminatory.\\

In summary, this post is not hateful based on the provided definition, but it is important to be aware of the context and potential implications of mentioning Jared Taylor.\\ \\

\bottomrule
\end{tabular}
\caption{Support Set Comparison (Latent Hatred vs FHM) - Examples of Latent Hatred's Effectiveness: Example 1}
\label{tab:cs2-p1-dem1}
\end{table*}

==> examples/cs2-p1-example2.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\#\#\# EXAMPLE 1}\\  
\textbf{Content:} A post containing 'this is white heritage . honor it'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: The post does not explicitly target a specific racial or ethnic group with harmful intent.\\

Derogatory Imagery/Language: There is no derogatory language or imagery used in the post.\\

Impact on Bias/Stereotypes: The post does not perpetuate harmful stereotypes or prejudices against any group. Instead, it appears to encourage the appreciation and preservation of cultural heritage, which is a positive sentiment. However, it is important to note that the term "white heritage" could be perceived as exclusionary or divisive, as it does not acknowledge the cultural heritage of other racial and ethnic groups.\\

In summary, this post is not hateful, but it may be perceived as exclusionary or divisive due to its focus on "white heritage."\\ \\

\textbf{\#\#\# EXAMPLE 2}\\  
\textbf{Content:} A post containing 'one monkey don't stop no show'\\
\textbf{Answer:} Hateful\\
\textbf{Rationale:} Targeted Group: The statement uses a derogatory term ("monkey") that is often used to demean and belittle people of African descent.\\

Derogatory Imagery/Language: The use of the term "monkey" is a racial slur that has a long history of being used to dehumanize and discriminate against people of African descent.\\

Impact on Bias/Stereotypes: This statement reinforces harmful stereotypes and prejudices against people of African descent, potentially inciting fear and hostility towards this group. It also contributes to a hostile and exclusionary environment for these individuals.\\

In summary, this post is hateful.\\ \\

\textbf{\#\#\# EXAMPLE 3}\\  
\textbf{Content:} A post containing 'block white hating crack monkey  i did .'\\
\textbf{Answer:} Hateful\\
\textbf{Rationale:} Targeted Group: The post targets individuals of a racial group (Black individuals) by using a derogatory term that is explicitly racist. It implies a dehumanizing and negative view of the targeted group.\\

Derogatory Imagery/Language: The term "crack monkey" is a highly offensive racial slur. It combines derogatory language with racist imagery, which is harmful and discriminatory.\\

Impact on Bias/Stereotypes: The post reinforces harmful stereotypes and prejudices against Black individuals. It perpetuates racial discrimination and contributes to a hostile and exclusionary environment by promoting dehumanization and negative racial stereotypes.\\

In summary, this post is hateful. \\ \\

\textbf{\#\#\# EXAMPLE 4}\\  
\textbf{Content:} A post containing 'these people should find it hateful and offensive to behead & honor kill . not you exposing those who behead \& honor kill .'\\
\textbf{Answer:} Hateful\\
\textbf{Rationale:} Targeted Group: The post targets individuals who practice certain religious or cultural traditions, such as those associated with honor killings and beheadings.\\

Derogatory Imagery/Language: The statement uses derogatory language by referring to these individuals as "these people," implying that they are a homogeneous group with negative characteristics.\\

Impact on Bias/Stereotypes: The post reinforces harmful stereotypes and prejudices against individuals who practice certain religious or cultural traditions, potentially inciting fear and hostility towards these groups. It also contributes to a divisive and exclusionary environment by suggesting that these practices are inherently wrong and should be condemned without understanding the cultural context.\\

In summary, this post is hateful.\\

\bottomrule
\end{tabular}
\caption{Support Set Comparison (Latent Hatred vs FHM) - Examples of Latent Hatred's Effectiveness: Example 2}
\label{tab:cs2-p1-dem2}
\end{table*}

==> examples/cs2-p2-example1.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\#\#\# EXAMPLE 1}\\  
\textbf{Content:} A meme with the caption, 'a woman sitting in a shopping cart with her legs up in the air', and overlay text, 'went to wal-mart and had a bit of fun'\\  
\textbf{Answer:} Not Hateful\\  
\textbf{Rationale:} Targeted Group: The meme does not target any specific group based on race, religion, ethnicity, gender, sexual orientation, disability, or other distinguishing characteristics.\\  

Derogatory Imagery/Language: The imagery in the meme is a woman sitting in a shopping cart in a playful manner, which does not contain any derogatory imagery or language towards any group.\\  

Impact on Bias/Stereotypes: The meme is a humorous portrayal of a woman finding joy and entertainment in an everyday activity and does not contribute to perpetuating negative biases, stereotypes, prejudice, discrimination, or inciting harm towards any particular group.\\  

In summary, the meme is not hateful.\\ \\  

\textbf{\#\#\# EXAMPLE 2}\\  
\textbf{Content:} A meme with the caption, 'a young woman wearing a hijab smiles at the camera', and overlay text, 'look! a beautiful muslim woman'\\
\textbf{Answer:} Not Hateful\\  
\textbf{Rationale:} Targeted Group: The meme does not explicitly target a specific racial or ethnic group, instead focusing on the woman's religious and cultural choice to wear a hijab.\\

Derogatory Imagery or Language: The text "look! a beautiful Muslim woman" does not contain derogatory language nor does it mock or demean the woman or Muslim women in general. Instead, it emphasizes her beauty.\\

Impact on Bias/Stereotypes: By emphasizing the woman's beauty, the meme does not contribute to perpetuating negative biases, stereotypes, prejudice, discrimination, or inciting harm towards Muslim women. Instead, it portrays a Muslim woman as normal and beautiful, countering negative stereotypes and promoting inclusivity.\\

In summary, the meme is not hateful.\\ \\

\textbf{\#\#\# EXAMPLE 3}\\  
\textbf{Content:} A meme with the caption, 'a woman with glasses and a purple shirt is sitting at a table with her hands together', and overlay text, 'me sitting at work thinking about what i'm going to eat for lunch'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: The meme does not directly target any specific group based on race, religion, ethnicity, gender, sexual orientation, disability, or other distinguishing characteristics.\\

Derogatory Imagery/Language: The meme does not contain any derogatory imagery or language. The woman in the meme is simply sitting and thinking about lunch.\\

Impact on Bias/Stereotypes: The meme does not contribute to perpetuating any negative bias, stereotypes, prejudice, discrimination, or inciting harm towards any specific group. It is a relatable and common scenario for many people, not associated with any harm or marginalization.\\

In summary, the meme is not hateful.\\ \\

\textbf{\#\#\# EXAMPLE 4}\\  
\textbf{Content:} A meme with the caption, 'a woman in a white dress sitting at a desk', and overlay text, 'this is my diary'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: There is no targeted group in this meme as it does not focus on race, religion, ethnicity, gender, sexual orientation, disability, or any other distinguishing characteristics.\\

Derogatory Imagery/Language: The meme is simply an image of a woman sitting at a desk without any derogatory imagery or language used.\\

Impact on Bias/Stereotypes: The meme does not contain any content that perpetuates bias, stereotypes, prejudice, discrimination, or incites harm towards any group. It is a humorous portrayal of a woman appearing to keep a diary, likely a reference to a historical figure such as Marie Tussaud. The meme does not contribute to any negative biases or stereotypes.\\

In summary, the meme is not hateful.\\ \\


\bottomrule
\end{tabular}
\caption{Support Set Comparison (Latent Hatred vs FHM) - Examples of FHM's Ineffectiveness: Example 1}
\label{tab:cs2-p2-dem1}
\end{table*}

==> examples/cs2-p2-example2.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{p{\linewidth}}
\toprule
\textbf{\#\#\# EXAMPLE 1}\\  
\textbf{Content:} A meme with the caption, 'a coffee maker with a cup of coffee', and overlay text, 'every man needs a decent coffee maker'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: The meme does not specifically target any particular group based on their race, religion, ethnicity, gender, sexual orientation, disability, or other distinguishing characteristics.\\

Derogatory Imagery/Language: The meme does not contain any derogatory imagery or language towards any group. The only content in the meme is a coffee maker and a cup of coffee, which is a non-controversial topic.\\

Impact on Bias/Stereotypes: The meme does not contribute to perpetuating negative biases, stereotypes, prejudice, discrimination, or inciting harm towards any specific group. It is a simple portrayal of a coffee maker and a cup of coffee, and there is no content that might be considered hostile or degrading towards any group. In summary, the meme is not hateful.\\ \\

\textbf{\#\#\# EXAMPLE 2}\\  
\textbf{Content:} A meme with the caption, 'a woman is making a cup of coffee in her kitchen', and overlay text, 'making decent coffee'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: There is no targeted group in this meme as it is not based on race, religion, ethnicity, gender, sexual orientation, disability, or other distinguishing characteristics.\\

Derogatory Imagery/Language: The imagery in the meme is a woman making coffee, which does not contain any derogatory imagery or language towards any group.\\

Impact on Bias/Stereotypes: The meme does not contain any content that perpetuates bias, stereotypes, prejudice, discrimination, or incites harm towards any group. It is simply a humorous portrayal of someone making coffee.\\

In summary, the meme is not hateful.\\ \\

\textbf{\#\#\# EXAMPLE 3}\\   
\textbf{Content:} A meme with the caption, 'a young girl in a white dress', and overlay text, 'no less beautiful'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: The meme does not specifically target a particular group based on race, religion, ethnicity, gender, sexual orientation, disability, or any other distinguishing characteristics.\\

Derogatory Imagery/Language: The meme does not contain any derogatory imagery or language.\\

Impact on Bias/Stereotypes: The meme does not contribute to perpetuating any negative bias, stereotypes, prejudice, discrimination, or inciting harm towards any specific group. It is simply expressing a positive sentiment about a young girl in a white dress, which is not hateful in any way. \\

In summary, the meme is not hateful.\\ \\

\textbf{\#\#\# EXAMPLE 4}\\  
\textbf{Content:} A meme with the caption, 'a woman in a white bikini top chopping food in a kitchen', and overlay text, 'the wife said we needed a new coffee maker, so i got one. the name is mr. coffee, the wife was amused'\\
\textbf{Answer:} Not Hateful\\
\textbf{Rationale:} Targeted Group: The meme does not specifically target any group based on race, religion, ethnicity, gender, sexual orientation, disability, or other distinguishing characteristics.\\

Derogatory Imagery or Language: There is no derogatory imagery or language used in the meme that could be considered hateful or discriminatory towards any group.\\

Impact on Bias/Stereotypes: The meme does not contribute to perpetuating any negative biases, stereotypes, prejudice, discrimination, or inciting harm towards any specific group. It is simply a humorous portrayal of a man introducing a new coffee maker while his wife reacts with amusement.\\

In summary, the meme is not hateful.\\

\bottomrule
\end{tabular}
\caption{Support Set Comparison (Latent Hatred vs FHM) - Examples of FHM's Ineffectiveness: Example 2}
\label{tab:cs2-p2-dem2}
\end{table*}
